Early-Learning Regularization Prevents Memorization of Noisy Labels

We propose a novel framework to perform classification via deep learning in the presence of noisy annotations. When trained on noisy labels, deep neural networks have been observed to first fit the training data with clean labels during an "early learning" phase, before eventually memorizing the examples with false labels. We prove that early learning and memorization are fundamental phenomena in high-dimensional classification tasks, even in simple linear models, and give a theoretical explanation in this setting. Motivated by these findings, we develop a new technique for noisy classification tasks, which exploits the progress of the early learning phase. In contrast with existing approaches, which use the model output during early learning to detect the examples with clean labels, and either ignore or attempt to correct the false labels, we take a different route and instead capitalize on early learning via regularization. There are two key elements to our approach. First, we leverage semi-supervised learning techniques to produce target probabilities based on the model outputs. Second, we design a regularization term that steers the model towards these targets, implicitly preventing memorization of the false labels. The resulting framework is shown to provide robustness to noisy annotations on several standard benchmarks and real-world datasets, where it achieves results comparable to the state of the art.

==> proof_lemma2.tex <==
\begin{align} 
\mathcal{R}(\param) := \log \left(1-\langle \vp^{[i]},\vq^{[i]} \rangle\right). 
\end{align}
we get the gradient of $\mathcal{R}$ is
\begin{align}
    \nabla \mathcal{R}(\param) & = \frac{1}{1-\langle \vp^{[i]},\vq^{[i]} \rangle} \nabla \left(1-\langle \vp^{[i]},\vq^{[i]} \rangle\right) \\
    & = \sum_{i=1}^n\frac{1}{1-\langle \vp^{[i]},\vq^{[i]} \rangle} \nabla \left(1-\frac{\langle e^{\func_{\vx^{[i]}}(\param)},\vq^{[i]} \rangle}{\sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}}\right)\\
    & =\sum_{i=1}^n\frac{-1}{1-\langle \vp^{[i]},\vq^{[i]} \rangle} \frac{\nabla\langle e^{\func_{\vx^{[i]}}(\param)},\vq^{[i]} \rangle \cdot \sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c} - \langle e^{\func_{\vx^{[i]}}(\param)},\vq^{[i]} \rangle\cdot \nabla  
    \sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}
    }{\left(\sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}\right)^2}\\
    & =\sum_{i=1}^n\frac{-\nabla \func_{\vx^{[i]}}(\param)}{1-\langle \vp^{[i]},\vq^{[i]} \rangle} 
    \frac{ e^{\func_{\vx^{[i]}}(\param)}\odot \vq^{[i]} \cdot \sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c} - \langle e^{\func_{\vx^{[i]}}(\param)},\vq^{[i]} \rangle\cdot 
    e^{\func_{\vx^{[i]}}(\param)}
    }{\left(\sum_{c=1}^C
    e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}\right)^2}\\
    & = \sum_{i=1}^n\frac{-\nabla \func_{\vx^{[i]}}(\param)}{1-\langle \vp^{[i]},\vq^{[i]} \rangle}\left(
    \frac{e^{\func_{\vx^{[i]}}(\param)}\odot \vq^{[i]}}{\sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}} - \frac{\langle e^{\func_{\vx^{[i]}}(\param)},\vq^{[i]} \rangle}{\sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}}\cdot  \frac{e^{\func_{\vx^{[i]}}(\param)}}{\sum_{c=1}^C e^{\left(\func_{\vx^{[i]}}(\param)\right)_c}}\right)\\
    & = \frac{-\nabla \func_{\vx^{[i]}}(\param)}{1-\langle \vp^{[i]},\vq^{[i]} \rangle}\left(\vp^{[i]}\odot \vq^{[i]} - \langle\vp^{[i]},\vq^{[i]}\rangle\cdot \vp^{[i]} \right)\\
    % & = \nabla \func_{\vx^{[i]}}(\param) \frac{\vp^{[i]}}{1-\langle \vp^{[i]},\vq^{[i]} \rangle}\odot \left (\langle \vp^{[i]},\vq^{[i]}  \rangle \odot \mathbf{1}   - \vq^{[i]} \right)\\
    & =  \nabla \func_{\vx^{[i]}}(\param) \frac{1}{1-\langle \vp^{[i]},\vq^{[i]} \rangle} \begin{bmatrix} \vp^{[i]}_1 \cdot \left( \langle\vp^{[i]},\vq^{[i]}\rangle - \vq^{[i]}_1\right)\\ \vdots \\ \vp^{[i]}_C\cdot \left( \langle\vp^{[i]},\vq^{[i]}\rangle - \vq^{[i]}_C\right) \end{bmatrix}\\
    & =  \nabla \func_{\vx^{[i]}}(\param) \frac{1}{1-\langle \vp^{[i]},\vq^{[i]} \rangle} \begin{bmatrix} \vp^{[i]}_1 \cdot \sum_{k=1}^C\left(\vq_k^{[i]}-\vq_1^{[i]}\right)\vp^{[i]}_k\\ \vdots \\  \vp^{[i]}_C \cdot \sum_{k=1}^C\left(\vq_k^{[i]}-\vq_C^{[i]}\right)\vp^{[i]}_k \end{bmatrix}\\
\end{align}

==> random.tex <==
Two classes from two $p$-dimensional Gaussian distributions  $\mathcal{N}(\mu_1, \Sigma)$ and $\mathcal{N}(\mu_2, \Sigma)$ with 
\begin{align}
    \mu_1 &= \left[\frac{1}{\sqrt{p}},\frac{1}{\sqrt{p}},\dots,\frac{1}{\sqrt{p}}\right],\\
    \mu_2 &= \left[-\frac{1}{\sqrt{p}},-\frac{1}{\sqrt{p}},\dots,-\frac{1}{\sqrt{p}}\right],\\
    \Sigma &= \text{diag}\left([0.01,0.01,\dots, 0.01]\right) .
\end{align}
\begin{align*}
    \mathcal{L}(\theta) = -\sum_{i=1}^n y_i\log s_i(\theta) - (1-y_i)\log (1-s_i(\theta)),
\end{align*}
where $s_i(\theta) = \frac{1}{1+e^{-x_i^T \theta}}$.
The gradient of the logistic regression is:
\begin{align}
    \frac{\partial \mathcal{L}}{\partial \theta} = \sum_{i=1}^n x_i(s_i-y_i).
\end{align}
The gradient of the proposed regularization:
\begin{align}
    \frac{\partial \mathcal{R}}{\partial \theta} = -\sum_{i=1}^n x_i\frac{(2q_i-1)s_i(1-s_i)}{q_i+s_i-2q_is_i}.
\end{align}
Together we have the gradient as :
\begin{align}
 \sum_{i=1}^n x_i\left[(s_i-y_i)-\beta \frac{(2q_i-1)s_i(1-s_i)}{q_i+s_i-2q_is_i}\right].
\end{align}

We would like the model to train on the label from original dataset as some of them can be correct, but also keep an eye on the model's predictions especially when the observed labels are not consistent with the predictions. Therefore we suggest a general framework to make the model, on hand, training on the prediction, on the other hand stay close to the model's prediction.
\begin{align}
    \mathcal{L} = \alpha\mathcal{L}_\text{CE}(s_\theta,y) + \beta \mathcal{R}(s_{\theta}, q),
    \label{eq:general_term}
\end{align}

Many previous works fall in to this framwork: Bootstrap , Symmetric entropy loss~\cite{wang2019symmetric}, Joint optimization\citet{tanaka2018joint,yi2019probabilistic}, the only difficulty is to choose $\mathcal{R}$. As the effective of $\mathcal{R}$ on training could be understand by seeing how it influence the activations, we thereby analysis the gradient of the loss respect to the activation:

\begin{align*}
    \frac{\partial \mathcal{R}(s,q)}{\partial a_j} &= \sum_{i\neq j} \left(\frac{\partial \mathcal{R}(s,q)}{\partial s_i}\cdot\frac{\partial s_i}{\partial a_j} \right) + \frac{\partial \mathcal{R}(s,q)}{\partial s_j}\cdot\frac{\partial s_j}{\partial a_j}\\
    & = -\sum_{i\neq j}\frac{\partial \mathcal{R}(s,q)}{\partial s_i}\cdot s_i s_j + \frac{\partial \mathcal{R}(s,q)}{\partial s_j}\cdot s_j(1-s_j)\\
    & = -\sum_{i}^c\frac{\partial \mathcal{R}(s,q)}{\partial s_i}\cdot s_i s_j + \frac{\partial \mathcal{R}(s,q)}{\partial s_j}\cdot s_j\\
    & =- s_j \left(\sum_i s_i \frac{\partial \mathcal{R}(s,q)}{\partial s_i} - \frac{\partial \mathcal{R}(s,q)}{\partial s_j} \right)\\
    & =- s_j \left[\sum_i s_i \left(\frac{\partial \mathcal{R}(s,q)}{\partial s_i} - \frac{\partial \mathcal{R}(s,q)}{\partial s_j} \right)\right]
\end{align*}

\section{KL divergence}

\begin{itemize}
\item Most widely used $\mathcal{R}$ is KL divergence, Cross Entropy
\item However, we observed that : higher $\beta$ The $q$ drives the learning process: the model is improving slowly. lower $\beta$ the noisy labels are fitted very fast: cannot prevent the model from memorizing the wrong labels. 
\item Whatever in between suffers a little both.
\item No reason to fit the value in $q$
\item when $p_j=q_j$, even though the $q$ still shows that the $j$ is the dominant class, the model will not improve on $j$
\end{itemize}

\section{Our Loss}
\begin{itemize}
   \item We want something maintain the correct prediction
   \item We want the gradient large when the confidence is large because as we showed before the confidence on the correct prediction is larger than incorrect predictions. 
   \item We proposed the loss:
   \begin{align}
\mathcal{R}_{\text{CE}}(\theta)  = 
 -\frac{1}{n}\sum_{i=1}^n\sum_{j=1}^c  q_{ij}\log s_{\theta}(j|\mathbf{x}_i),
\label{eq:boot_loss}
\end{align}
\item where $\frac{\partial\mathcal{R}}{\partial a_j}$ is proportional to $ \sum_{i=1}^c(q_i-q_j)p_i$ which will be negative when $q_j$ is dominant i.e. $q_j\geq q_i\; \forall i$ regardless of the value of $p$. Moreover, the magnitude is large when $q$ is confident. 
   
\end{itemize}


==> sec_experimets.tex <==
\section{Experiments}
We evaluate the proposed methodology on two standard benchmarks with simulated label noise, CIFAR-10 and CIFAR-100~\cite{krizhevsky2009learning}, and two real-world datasets, Clothing1M~\cite{xiao2015learning} and WebVision~\cite{li2017webvision}. In addition, we perform an ablation study on CIFAR-10. For CIFAR-10 and CIFAR-100 we simulate label noise by randomly flipping a certain fraction of the labels in the training set following a \textit{symmetric} uniform distribution (as in Eq.~(\ref{eq:sym_noise})), as well as a more realistic \textit{asymmetric} class-dependent distribution, as in~\cite{patrini2017making}. Clothing1M consists of 1 million training images collected from online shopping websites with labels generated from surrounding text. Its noise level is estimated at $38.5\%$~\cite{song2019prestopping}. For ease of comparison to previous works~\cite{jiang2017mentornet,chen2019understanding}, we consider first 50 categories to select a subset of WebVision with approximately 66k images crawled from Google image search.
The noise level of WebVision is estimated at $20\%$~\cite{li2017webvision}. Table~\ref{tab:data_describ} in the supplementary material reports the image size, and the number of examples in the training, validation and test splits for each of the data sets. 

In our experiments, we prioritize making our results comparable to the existing literature. We therefore use the same preprocessing, architectures, and training procedures as previous methods. The details are described in Section~\ref{sec:experiments_appendix} of the supplementary material. We focus mainly on two variants of the proposed approach: ELR with temporal ensembling, which we call ELR, and ELR with temporal ensembling, weight averaging, two networks, and mixup data augmentation, which we call ELR+. For completeness, we include a detailed description of both options in Section~\ref{sec:ELR_ELR+} of the supplementary material. In Section~\ref{} we report the results of an ablation study that evaluates the contribution of each element.

==> sec_results.tex <==
\section{Results}
Table~\ref{tab:results_loss_correction_methods} shows results of loss correction methods
\input{table/loss_correction}
\begin{itemize}
    \item improvements and analysis on the results.
\end{itemize}

\input{table/clothing1m}
\subsection{Combine with other methods}
\input{NoisyLabel/table/combine}
\input{NoisyLabel/table/webvision}
\input{NoisyLabel/table/ablation_40}
\subsection{Ablation Studies}
To asses the importance of various aspects of the model, we run experiments on CIFAR10 with 60\% symmetric noisy label, varying one or a few hyperparameters at a time while keeping the other fixed.
\subsubsection{Sensitivity to aggregation}
we select the parameter $\beta$ from set $\{0.0, 0.01, 0.1,\; 0.3,\; 0.5,\; 1.0\}$. Note that when $\alpha = 1.0$, the immediate prediction is used. The method is quite stable across different values of $\beta$.    
\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\linewidth]{NoisyLabel/images/ablation_agg.png}
    \includegraphics[width=0.45\linewidth]{NoisyLabel/images/ablation_existingapproaches.png}
    \includegraphics[width=0.45\linewidth]{NoisyLabel/images/ablation_coef.png}
    \includegraphics[width=0.45\linewidth]{NoisyLabel/images/ablation_mixup.png}
    \label{fig:ablation}
    \caption{\carlos{Remove top right. Put 3 in a row. 50\%-90\%. Put this in the appendix and describe it.}}
\end{figure}
\subsubsection{combining existing approaches}
\textbf{Mixup}

\textbf{Mean Teacher}

\textbf{Mutual Mean Teacher}

==> table/algorithm.tex <==
\begin{algorithm}[!t]
	
	\DontPrintSemicolon
	\small
	\textbf{Input:} $\theta^{(1)}$ and $\theta^{(2)}$, training dataset $(\mathcal{X},\mathcal{Y})$, aggregation parameter $\alpha$, regularization coefficient $\lambda$, $\mathrm{Beta}$ distribution parameter $\beta$ for $\mathrm{MixUp}$. \\

% 	$\theta^{(1)},\theta^{(2)}=\mathrm{WarmUp}(\mathcal{X},\mathcal{Y},\theta^{(1)},\theta^{(2)})$ \tcp*{standard training (with confidence penalty)}
	\While{$e<\mathrm{MaxEpoch}$}    
	{	
	\For( \tcp*[f]{train the two networks one by one}) {$k=1,2$}    
    {

		\For {$\mathrm{iter}=1$ \KwTo $\mathrm{num\_iters}$}
		{
			From $\mathcal{X}^{(k)}$, draw a mini-batch $\mathcal{B} = \{(x_i,y_i, q_i);i\in(1,...,|B|)\}$ \\
			$\mathcal{B} = \mathrm{MixUp}(\mathcal{B})$ \tcp*[f]{Apply MixUp to the mini-batch}\\
			\For{$i=1$ \KwTo $B$}\\
			{
				${q}^{(k)}_{i}=p_{MT}(x_i; \theta^{(k)}) \tcp*{average the predictions across augmentations of $x_b$}
				p
			}
			$\hat{\mathcal{X}}=\{(\hat{x}_{b,m},\hat{y}_b);b\in(1,...,B),m\in(1,...,M)\}$	\tcp*{augmented labeled mini-batch}
			$\hat{\mathcal{U}}=\{(\hat{u}_{b,m},q_{b});b\in(1,...,B),m\in(1,...,M)\}$	\tcp*{augmented unlabeled mini-batch}
	        $\mathcal{L}_\mathcal{X},\mathcal{L}_\mathcal{U}=\mathrm{MixMatch}(\hat{\mathcal{X}},\hat{\mathcal{U}})$ \tcp*{apply MixMatch}
			$\mathcal{L}=\mathcal{L}_\mathcal{X}+\lambda_u \mathcal{L}_\mathcal{U}+\lambda_r \mathcal{L}_\mathrm{reg}$ \tcp*{total loss}
			$\theta^{(k)}=\mathrm{SGD}(\mathcal{L},\theta^{(k)})$  \tcp*{update model parameters}
	    }
	}
	}
	\caption{\small Mutual Mean Teacher. Line 4-8: co-divide; Line 17-18: label co-refinement; Line 20: label co-guessing.}
	\label{alg:dividemix}
	
\end{algorithm}

==> table/animal.tex <==
\begin{table}
\footnotesize
\begin{center}
\begin{tabular}{c|c|c}
\hline
Model & Method & Test Error\\
\hline
\multirow{7}{*}{VGG19}&Cross-Entropy & 79.2\\
&Active Bias & 80.0 \\
&Co-teaching & 80.1\\
&Co-teaching+ & 77.6\\
&SELFIE & 81.4 \\
&Prestopping & 81.9\\
&Prestopping + & 82.2\\
&Ours & 84.4(Not tune yet)\\
\hline
\end{tabular}
\end{center}
\caption{Accuracy (\%) of different models on ANIMAL-10N.}
\end{table}

==> table/clothing1m.tex <==
% \begin{table}
% \begin{center}
% \begin{tabular}{c|c|c}
% \toprule
% Architecture &Method & Test Accuracy\\
% \midrule
% \multirow{10}{*}{\shortstack{ResNet-50 \\(pretrained)}}& CE& 69.10\\
% &Bootstrap~\cite{reed2014training} & 68.94\\
% &Forward~\cite{patrini2017making} & 69.84\\
% &GCE~\cite{zhang2018generalized} &69.75\\
% &SL~\cite{wang2019symmetric} & 71.02\\
% &Joint-Optim~\cite{tanaka2018joint} & 72.16\\
% &PENCIL~\cite{yi2019probabilistic} & 73.49\\
% &DivideMix~\cite{li2020dividemix} & 74.76\\
% \cmidrule{2-3}
% &ELR (proposed) & 72.87\\
% &ELR+ (proposed)& \textbf{74.81}\\
% \bottomrule
% \end{tabular}
% \end{center}
% \caption{Comparison of test accuracy different methods in test accuracy (\%) on real-world noisy dataset Clothing 1M }
% \label{tab:Clothing1M}
% \vspace{-2mm}
% \end{table}


\begin{table}
\begin{center}
 \resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
CE&
Bootstrap~\cite{reed2014training} & 
Forward~\cite{patrini2017making} & 
GCE~\cite{zhang2018generalized} &
SL~\cite{wang2019symmetric} &
Joint-Optim~\cite{tanaka2018joint} &
% PENCIL~\cite{yi2019probabilistic} &
DivideMix~\cite{li2020dividemix} &
ELR  &
ELR+ \\
\midrule
69.10 & 68.94 & 69.84 & 69.75 & 71.02 & 72.16  & 74.76 & 72.87& \textbf{74.81}\\
\bottomrule
\end{tabular}}
\end{center}

\caption{Comparison of test accuracy different methods in test accuracy (\%) on real-world noisy dataset Clothing 1M }
\label{tab:Clothing1M}

\vspace{-2mm}
\end{table}

==> table/combine.tex <==
% \begin{table}[h]
% \begin{center}
% \begin{tabular}{c|c|cccc}
% \hline
% \multirow{2}{*}{Architecture} & \multirow{2}{*}{Methods} & \multicolumn{4}{c}{\textit{Symm}} \\
%  & & 20 & 50 & 80 & 90\\
% \hline
% \multirow{9}{*}{PreActResNet-18}  & CE & 86.8 & 79.4 &62.9 & 42.7 \\
% & Bootstrap & 86.8 & 79.48 &63.3 & 42.9 \\
% & Co-teaching+ & 89.5 & 85.7 & 67.4 & 47.9\\
% & Mixup & 95.6 & 87.1 & 71.6 & 52.2\\
% & P-correction & 92.4 & 89.1 & 77.5 & 58.9\\
% & Meta-Learning & 92.9 & 89.3 & 77.4 & 58.7\\
%  & M-correction & 94.0 & 92.0 & 86.8 & 69.1\\
%  &DivideMix & 96.1 & 94.6 & 93.2 & 76.0\\
% & ELR+++* & 94.6 & 93.8 & 91.1 & 75.8\\
% \hline
% \end{tabular}
% \end{center}
% \caption{Comparison of performance of the state of the art methods in test accuracy (\%) on CIFAR-10 with symmetric noise. Note that previous methods choose the best test accuracy to report their results, where we report our results using the model with highest validation accuracy. *we use less training data and report results of most accurate model from the validation set.}
% \label{tab:MMT}
% \vspace{-2mm}
% \end{table}


\begin{table}[t]
\begin{center}
\begin{threeparttable}
\resizebox{\linewidth}{!}{
\begin{tabular}{c|c|c|c|c|c|c|c|c}
\toprule
\textit{Symm}&
CE & 
Bootstrap~\cite{reed2014training} & 
Co-teaching+~\cite{han2018co} & 
Mixup~\cite{zhang2017mixup} &
PENCIL~\cite{yi2019probabilistic} & 
MD-DYR-SH~\cite{Arazo2019unsup} &
DivideMix~\cite{li2020dividemix} & 
ELR+\tnote{$\diamond$} \\
\midrule
20\% & 86.8 & 86.8 & 89.5 & 95.6 & 92.4 & 94.0 & $\bf{96.1}$ & 94.6\\
40\% & 79.4 & 79.5 & 85.7 & 87.1 & 89.1 & 92.0 & $\textbf{94.6}$ & 93.8 \\
80\% & 62.9 & 63.3 & 67.4 & 71.6 & 77.5 & 86.8 & $\textbf{93.2}$ & 91.1\\
90\% & 42.7 & 42.9 & 47.9 & 52.2 & 58.9 & 69.1 & $\textbf{76.0}$ & 75.8\\
\bottomrule
\end{tabular}}
\begin{tablenotes}\footnotesize
\item[$\diamond$] \textit{Results on best validation model. }
\end{tablenotes}
\end{threeparttable}
\end{center}
\caption{Comparison of performance of the state of the art methods in test accuracy (\%) on CIFAR-10 with symmetric noise. Note that previous methods choose the best test accuracy to report their results, where we report our results using the model with highest validation accuracy. *we use less training data and report results of most accurate model from the validation set.}
\label{tab:MMT}
\vspace{-2mm}
\end{table}

==> table/loss_correction.tex <==

\begin{table}
\footnotesize
\begin{center}
\begin{threeparttable}
\begin{tabular}{c|c|cccc|cccc}
\toprule
\multirow{2}{*}{\shortstack{Datasets\\(Architecture)}} & \multirow{2}{*}{Methods} & \multicolumn{4}{c|}{\textit{Symmetric label noise}}&\multicolumn{4}{c}{\textit{Asymmetric label noise}} \\
 & & 20\% & 40\%  & 60\% & 80\%  & 10\% & 20\% & 30\% & 40\%\\
\midrule
\multirow{7}{*}{\shortstack{CIFAR10\\(ResNet34)}}  & Cross entropy & 86.98 & 81.88 & 74.14 & 53.82 & 90.69 & 88.59 & 86.14 & 80.11 \\
%MAE & 83.72 & 67.00 & 64.21 & 38.63 & 82.61 & 52.93 & 50.36 & 45.52\\
  %& Forward $T$ & 88.63 & 85.07 & 79.12 & 64.30 & 91.32 & 90.35 & 89.25 & 88.12\\
   & Bootstrap~\cite{Reed2015TrainingDN}& 86.23 & 82.23 & 75.12 & 54.12  & 90.32 & 88.26 & 86.57 & 81.21\\
 & Forward~\cite{patrini2017making}& 87.99 & 83.25 & 74.96 & 54.64  & 90.52 & 89.09 & 86.79 & 83.55\\
  & GSE~\cite{zhang2018generalized}& 89.83 & 87.13  & 82.54 & 64.07 & 90.91 & 89.33 & 85.45 & 76.74\\
& SL~\cite{Wang2019SymmetricCE} & 89.83 & 87.13 & 82.81 & 68.12 & 91.72 & 90.44 & 88.48 & 82.51 \\
 & ELR & \textbf{92.16} & \textbf{89.25} & \textbf{86.34} & \textbf{75.32}  &\textbf{93.27} & \textbf{93.52} & \textbf{91.89} & \textbf{91.12} \\
  & ELR\tnote{$\star$} & \textbf{94.23} & \textbf{91.43} & \textbf{88.87} & \textbf{82.59}& \textbf{94.57} & \textbf{93.28} & \textbf{92.70} & \textbf{91.35} \\
\midrule
\multirow{7}{*}{\shortstack{CIFAR100\\(ResNet34)}} & Cross entropy & 58.72 & 48.20 & 37.41 & 18.10 &  66.54 & 59.20 & 51.40 & 42.74 \\
 & Bootstrap~\cite{Reed2015TrainingDN}& 58.27 & 47.66 & 34.68  & 21.64  & 67.27 & 62.14 & 52.87 & 45.12\\
  & Forward~\cite{patrini2017making} & 39.19 & 31.05 & 19.12 & 8.99 & 45.96 & 42.46 & 38.13 & 34.44\\
  & GSE~\cite{zhang2018generalized} & 67.61 & 62.64 & 54.04 & 29.60 & 68.86 & 66.59 & 61.87 & 47.66\\
  & SL~\cite{Wang2019SymmetricCE} & 70.38 & 63.27 & 54.82 & 27.91 & 73.12 & 72.56 &72.12 & 69.32 \\
  & ELR  & \textbf{73.21} & \textbf{65.21} & \textbf{59.48} & \textbf{31.21} & 
                     \textbf{74.20} & \textbf{74.03} & \textbf{73.71} & \textbf{72.26}\\
  & ELR\tnote{$\star$}  & \textbf{73.68} & \textbf{67.53} & \textbf{61.05} & \textbf{32.27} & 
                      \textbf{74.52} & \textbf{74.20} & \textbf{73.82} & \textbf{72.73}\\
\bottomrule
\end{tabular}
\begin{tablenotes}\footnotesize
\item[$\star$] \textit{Results with cosine annealing learning rate. }
\end{tablenotes}
\end{threeparttable}
\end{center}

\caption{Comparison with existing methods on CIFAR-10 and CIFAR-100 with symmetric and asymmetric label noise. The bootstrap and SL methods were reimplemented using publicly available code, the rest of results are taken from~\cite{zhang2018generalized}.}
\label{tab:results_loss_correction_methods}
\vspace{-2mm}
\end{table}

==> table/webvision.tex <==
% \begin{table}[h]
% 	\centering
% 	\small
% 	\begin{tabular}	{l |c|c|c|c|c }
% 		\toprule	 	
% 			\multirow{2}{*}{Architecture} &	\multirow{2}{*}{Method}  & \multicolumn{2}{c|}{WebVision} & \multicolumn{2}{c}{ILSVRC12}\\
% 			\cmidrule{3-6}
% 		&	& top1 & top5& top1 & top5\\
% 			\midrule			
% 		\multirow{9}{*}{Inception-ResNet-v2} &	F-correction & 61.12 & 82.68&  57.36 &82.36\\	
% 			& Decoupling & 62.54 &84.74& 58.26 &82.26\\
% 			& D2L &62.68 &84.00&  57.80 &81.36\\
% 			& MentorNet &63.00 &81.40&  57.80 &79.92\\	
			
% 			& Co-teaching&63.58 &85.20&   61.48 &84.70\\			
% 			& Iterative-CV 	&  65.24 &85.34&  61.60 &84.98\\	
% 			& DivideMix & 77.32 & 91.64 & 75.20 & 90.84\\
% 			\cmidrule{2-6}
% 			& ELR &76.26 &91.26& 68.71 &87.64\\
% 			& ELT+++ & 77.78 &91.68& 71.25 & 89.68\\
% 		\bottomrule
% 	\end{tabular}
% 	%}
% 	\caption
% 		{
% 		%\small	
% 		Comparison with state-of-the-art methods trained on (mini) WebVision dataset. Numbers denote top-1 (top-5) accuracy (\%) on the WebVision validation set and the ImageNet ILSVRC12 validation set.
% 		Results for baseline methods are copied from~\cite{Chen_ICML_2019}.
% 		}
% 	\label{tbl:webvision}

% \end{table}	

\begin{table}[h]
	\centering
	\resizebox{\linewidth}{!}{
	\begin{tabular}	{c|c|c|c|c|c|c|c|c}
		\toprule	 	
			& & 
			  D2L~\cite{ma2018dimensionality} &
			  MentorNet~\cite{jiang2017mentornet}&
			  Co-teaching~\cite{han2018co} &	
			  Iterative-CV~\cite{wang2018iterative}	&	
			  DivideMix~\cite{li2020dividemix}&
			  ELR &
			  ELR+ \\
			  \midrule			
		\multirow{2}{*}{WebVision} &top1 &  62.68 & 63.00 & 63.58 & 65.24 & 77.32 & 76.26 & 77.78\\
		& top5  & 84.00 & 81.40 & 85.20 & 85.34 & 91.64 & 91.26 & 91.68\\
		 \midrule	
		 \multirow{2}{*}{ILSVRC12} &top1  & 57.80 & 57.80 & 61.48 & 61.60 & 75.20 & 68.71 & 70.89\\
		& top5  & 81.36 & 79.92 & 84.70 & 84.98 & 90.84 & 87.84 & 89.76\\
		 
			
		\bottomrule
	\end{tabular}}
	%}
	\caption
		{
		%\small	
		Comparison with state-of-the-art methods trained on (mini) WebVision dataset. Numbers denote top-1 (top-5) accuracy (\%) on the WebVision validation set and the ImageNet ILSVRC12 validation set.
		Results for baseline methods are copied from~\cite{Chen_ICML_2019}.
		}
	\label{tbl:webvision}

\end{table}	
